Graph Reconstruction from Connected Triples

The problem of graph reconstruction has been studied in its various forms over the years. In particular, the Reconstruction Conjecture, proposed by Ulam and Kelly in 1942, has attracted much research attention and yet remains one of the foremost unsolved problems in graph theory. Recently, Bastide, Cook, Erickson, Groenland, Kreveld, Mannens, and Vermeulen proposed a new model of partial information, where we are given the set of connected triples T_3, which is the set of 3-subsets of the vertex set that induce connected subgraphs. They proved that reconstruction is unique within the class of triangle-free graphs, 2-connected outerplanar graphs, and maximal planar graphs. They also showed that almost every graph can be uniquely reconstructed from their connected triples. However, little is known about other classes of non-triangle-free graphs within which reconstruction can occur uniquely, nor do we understand what kind of graphs can be uniquely reconstructed from their connected triples without assuming anything about the classes of graphs to which they belong. The main result of this paper is a complete characterization of all graphs that can be uniquely reconstructed from their connected triples T_3. We also show that reconstruction from T_3 is unique within the class of regular planar graphs, 5-connected planar graphs, certain strongly regular graphs, and complete multi-partite graphs, whereas it is not unique for the class of k-connected planar graphs with k less or equal to 4, Eulerian graphs, or Hamiltonian graphs.

==> Figure1.tex <==
\begin{asy}
size(12cm);
usepackage("amsmath");
usepackage("amssymb");
dotfactor *= 1.5;
dot((0,0));

pen highlight = opacity(0.2)+red+7;

pair A(real i) { return dir(30+60*i); }
for (int i=0; i<6; ++i) {
  dot(A(i));
  draw(A(i)--A(i+1));
  if (i != 0) { draw((0,0)--A(i)); }
}
label("$6$", dir(90), dir(90));
label("$1$", dir(150), dir(150));
label("$2$", dir(210), dir(210));
label("$3$", dir(270), dir(270));
label("$7$", (0,0), dir(30));
draw(dir(30)..(1.4*dir(90))..dir(150));
draw(dir(30)..(1.4*dir(-30))..dir(-90));
draw(dir(30)..(1.7*dir(-60))..dir(210));
path p = dir(90)--dir(150)--dir(210)--dir(270)--dir(330)--cycle;
draw(p, black+2);
draw(p, highlight);

transform t = shift(3,0);
add(t*currentpicture);
label("$\boxed{5}$", dir(30), dir(30), red);
label("$\boxed{4}$", dir(-30), dir(0), red);
label("$\boxed{4}$", t*dir(30), dir(30), red);
label("$\boxed{5}$", t*dir(-30), dir(0), red);

picture b;
pair B(real i) { return dir(112.5+45*i); }
for (int i=0; i<8; ++i) {
  dot(b, B(i));
  draw(b, B(i)--B(i+1));
  if (i != 7) {
  draw(b, (0,0)--B(i));
  }
}
path q = B(8)--B(1)--B(2)--B(3)--B(4)--B(5)--B(6)--B(8);
draw(b, q, black+2);
draw(b, q, highlight);
label(b, "$\boxed{n-1}$", B(7), 2.5*dir(5), red);
label(b, "$\boxed{n-2}$", B(6), B(6), red);
label(b, "$1$", B(1), B(1));
label(b, "$2$", B(2), B(2));
label(b, "$n$", B(8), B(8));
dot(b, rotate(10)*"$n+1$", (0,0), 2*B(7));
draw(b, B(7)..(2.3*B(6))..B(5));
draw(b, B(7)..(2.6*B(6))..B(4));
draw(b, B(7)..(1.3*B(8))..B(1));
draw(b, B(7)..(1.7*B(8.5))..B(2));
draw(b, B(7)..(2*B(1))..B(3));
label(b, "$\boxed{n-1} \longleftrightarrow \boxed{n-2}$", (0,-1.4), red);
add(shift(1.5,-3.5)*b);
\end{asy}

==> Figure2.tex <==
\begin{asy}
size(9cm);
dotfactor *= 1.5;

void dotpath(picture pic, path p) {
  draw(pic, p);
  for (int i=0; i<size(p); ++i) {
    dot(pic, point(p, i));
  }
}

picture p1, p2, p3, p4, p5, p6, p7, p8, p9;
dotpath(p1, (2*dir(150)-dir(270))--dir(150)--dir(270)--dir(30)--(2*dir(30)-dir(270)));
draw(p1, dir(150)--dir(30));
add(scale(0.7)*p1);
label("Bull graph", 2*dir(90), fontsize(9pt));

dotpath(p2, 2*dir(135)--dir(135)--dir(225)--dir(315)--dir(45)--2*dir(45));
draw(p2,dir(135)--dir(45));
add(shift(3.5,0)*p2);

dotpath(p3, dir(90)--dir(162)--dir(234)--dir(306)--dir(18)--dir(90)--dir(90)*2);
draw(p3,dir(162)--dir(18));
add(shift(7,0)*p3);

dotpath(p4, dir(210)--dir(150)--dir(90)--dir(30)--dir(330));
dotpath(p4, dir(90)--dir(90)*2);
add(shift(10.5,0)*p4);

dotpath(p5, dir(30)--dir(90)--dir(150)--dir(210)--dir(270)--dir(330)--dir(30)--(dir(30)+dir(0))
  --(dir(30)+dir(0)+dir(270))--(dir(30)+dir(0)+2.5*dir(270)));
dotpath(p5, dir(270)--2*dir(270)--(1.5*dir(270)+dir(-30))--(dir(30)+dir(0)+2.5*dir(270))
  --(dir(30)+dir(0)+dir(270)));
draw(p5, dir(330)--(dir(330)+dir(0)));
add(shift(13.5,1)*p5);

for (int i=0; i<3; ++i) {
  dotpath(p6, dir(90+120*i)--2.5*dir(90+120*i));
  draw(p6, dir(90+120*i)--dir(210+120*i));
}
add(shift(1,-4)*scale(0.7)*p6);

dotpath(p7, (dir(225)+dir(270))--dir(225)--dir(135)--dir(45)--dir(-45)--(dir(-45)+dir(270)));
draw(p7, dir(225)--dir(315)--dir(135));
add(shift(5,-3)*p7);

dotpath(p8, dir(0)--dir(60)--dir(120)--dir(180)--dir(240)--dir(300)--cycle);
dotpath(p8, dir(0)--(1.9*dir(0)));
dotpath(p8, dir(120)--(1.9*dir(120)));
dotpath(p8, dir(180)--(1.9*dir(180)));
dotpath(p8, dir(240)--(1.9*dir(240)));
add(shift(9.5,-4)*p8);

dotpath(p9, dir(0)--dir(60)--dir(120)--dir(180)--dir(240)--dir(300)--dir(0)--dir(180));
add(shift(14,-4)*p9);
\end{asy}

==> Figure3.tex <==
\begin{asy}
size(13cm);
dotfactor *= 1.5;

pen de = dashed;
real r = 0.25;
real k = 2.3;

void mainedge(picture pic, pair v, pair w) {
  draw(pic, v--w, red+1.5);
  pair v1 = v+dir(90)*dir(w-v)*r;
  pair v2 = v-dir(90)*dir(w-v)*r;
  pair w1 = w+dir(90)*dir(v-w)*r;
  pair w2 = w-dir(90)*dir(v-w)*r;
  filldraw(pic, v1--w2..(w+r*dir(w-v))..w1--v2..(v+r*dir(v-w))..v1--cycle,
    opacity(0.1)+yellow, red);
}

picture p1, p2, p3, p4, p5, p6;
draw(p1, dir(90)--dir(330), de);
draw(p1, dir(210)--dir(330));
draw(p1, dir(90)--(k*dir(90)));
mainedge(p1, dir(90), dir(210));
dot(p1, dir(210));
dot(p1, "$v_2$", dir(330), dir(-90));
dot(p1, dir(90));
dot(p1, "$v_1$", k*dir(90), dir(90));
label(p1, "$u$", dir(90), dir(45)*2, red);
label(p1, "$v$", dir(210), dir(-90)*2, red);
add(p1);

draw(p2, dir(210)--dir(90)--dir(330));
draw(p2, dir(210)--dir(330), de);
mainedge(p2, dir(90), k*dir(90));
dot(p2, "$v_1$", dir(210), dir(-90));
dot(p2, "$v_2$", dir(330), dir(-90));
dot(p2, dir(90));
dot(p2, k*dir(90));
label(p2, "$u$", k*dir(90), dir(90)*2, red);
label(p2, "$v$", dir(90), dir(0)*2, red);
add(shift(3,0)*p2);

draw(p3, dir(90)--dir(180)--dir(270)--dir(0)--dir(90)--(k*dir(90)));
draw(p3, dir(180)--dir(0), de);
mainedge(p3, dir(180), dir(270));
dot(p3, "$v_3$", dir(0), dir(0));
dot(p3, "$v_2$", dir(90), dir(45));
dot(p3, dir(180));
dot(p3, dir(270));
dot(p3, "$v_1$", k*dir(90), dir(90));
label(p3, "$u$", dir(180), dir(180)*2, red);
label(p3, "$v$", dir(270), dir(-90)*2, red);
add(shift(6,0)*p3);

draw(p4, dir(90)--(2*dir(90))--(3*dir(90)));
draw(p4, dir(210)--dir(90)--dir(330));
draw(p4, dir(210)--dir(330), de);
mainedge(p4, 2*dir(90), 3*dir(90));
dot(p4, "$v_2$", dir(210), dir(-90));
dot(p4, "$v_3$", dir(330), dir(-90));
dot(p4, "$v_1$", dir(90), dir(0));
dot(p4, 2*dir(90));
dot(p4, 3*dir(90));
label(p4, "$u$", 3*dir(90), dir(0)*2, red);
label(p4, "$v$", 2*dir(90), dir(0)*2, red);
add(shift(9,-0.5)*p4);

transform t = scale(1.2);
draw(p5, t*(dir(180)--dir(135)--dir(90)--dir(45)));
draw(p5, t*(dir(45)--dir(180)--dir(0)), de);
mainedge(p5, t*dir(45), t*dir(0));
dot(p5, t*dir(0));
dot(p5, t*dir(45));
dot(p5, "$v_3$", t*dir(90), dir(90));
dot(p5, "$v_2$", t*dir(135), dir(110));
dot(p5, "$v_1$", t*dir(180), dir(-90));
label(p5, "$u$", t*dir(45), dir(90)*2, red);
label(p5, "$v$", t*dir(0), dir(-90)*2, red);
add(shift(12,-0.5)*p5);

draw(p6, dir(-54)--dir(18)--dir(162)--dir(90));
draw(p6, dir(162)--dir(234));
draw(p6, dir(18)--dir(90), de);
mainedge(p6, dir(234), dir(306));
dot(p6, "$v_2$", dir(90), dir(90));
dot(p6, "$v_1$", dir(162), dir(132));
dot(p6, dir(234));
dot(p6, dir(306));
dot(p6, "$v_3$", dir(18), dir(48));
label(p6, "$u$", dir(234), dir(-90)*2, red);
label(p6, "$v$", dir(306), dir(-90)*2, red);
add(shift(15,0)*p6);

for (int i=1; i<=6; ++i) {
  label("$\mathcal{F}_" + (string)i + "$", (3*i-3,-2.5));
}
\end{asy}

==> Figure4.tex <==
\begin{asy}
size(10cm);
dotfactor *= 1.5;

pen de = dashed;
real r = 0.15;
real k = 2.3;

void mainedge(picture pic, pair v, pair w) {
  draw(pic, v--w, red+1.5);
  pair v1 = v+dir(90)*dir(w-v)*r;
  pair v2 = v-dir(90)*dir(w-v)*r;
  pair w1 = w+dir(90)*dir(v-w)*r;
  pair w2 = w-dir(90)*dir(v-w)*r;
  filldraw(pic, v1--w2..(w+r*dir(w-v))..w1--v2..(v+r*dir(v-w))..v1--cycle,
    opacity(0.1)+yellow, red);
}

picture p1, p2, p3, p4, p5, p6;
draw(p1, dir(90)--dir(330), de);
draw(p1, dir(210)--dir(330));
draw(p1, dir(90)--(k*dir(90)));
mainedge(p1, dir(90), dir(210));
dot(p1, dir(210));
dot(p1, dir(330));
dot(p1, dir(90));
// dot(p1, "$\alpha$", k*dir(90), dir(0));
dot(p1, k*dir(90));
label(p1, "$\mathcal{F}_1$", (0,-1.3), dir(-90));
add(p1);

draw(p2, dir(210)--dir(90)--dir(330));
draw(p2, dir(210)--dir(330), de);
mainedge(p2, dir(90), k*dir(90));
dot(p2, dir(210));
dot(p2, dir(330));
dot(p2, dir(90));
dot(p2, k*dir(90));
label(p2, "$\mathcal{F}_2$", (0,-1.3), dir(-90));
add(shift(3,0)*p2);

draw(p3, dir(90)--dir(180)--dir(270)--dir(0)--dir(90)--(k*dir(90)));
draw(p3, dir(180)--dir(0), de);
mainedge(p3, dir(180), dir(270));
dot(p3, dir(0));
dot(p3, dir(90));
dot(p3, dir(180));
dot(p3, dir(270));
dot(p3, k*dir(90));
label(p3, "$\mathcal{F}_3$", (0,-1.3), dir(-90));
add(shift(6,0)*p3);

draw(p4, dir(90)--(2*dir(90))--(3*dir(90)));
draw(p4, dir(180)--dir(90)--dir(0));
draw(p4, dir(180)--dir(0), de);
mainedge(p4, 2*dir(90), 3*dir(90));
dot(p4, dir(0));
dot(p4, dir(90));
dot(p4, dir(180));
dot(p4, 2*dir(90));
dot(p4, 3*dir(90));
label(p4, "$\mathcal{F}_4$", (0,-0.8), dir(-90));
add(shift(9,-0.5)*p4);


draw(p5, dir(180)--dir(135)--dir(90)--dir(45));
draw(p5, dir(45)--dir(180)--dir(0), de);
mainedge(p5, dir(45), dir(0));
dot(p5, dir(0));
dot(p5, dir(45));
dot(p5, dir(90));
dot(p5, dir(135));
dot(p5, dir(180));
label("$\mathcal{F}_5$", (2,-4.8), dir(-90));
add(shift(2,-4.3)*scale(1.4)*p5);

draw(p6, dir(-54)--dir(18)--dir(162)--dir(90));
draw(p6, dir(162)--dir(234));
draw(p6, dir(18)--dir(90), de);
mainedge(p6, dir(234), dir(306));
dot(p6, dir(90));
dot(p6, dir(162));
dot(p6, dir(234));
dot(p6, dir(306));
dot(p6, dir(18));
label("$\mathcal{F}_6$", (7,-4.8), dir(-90));
add(shift(7,-3.5)*p6);
\end{asy}

==> Figure5.tex <==
\begin{asy}
fillRu("$u$");
fillRv("$v$");
fillRw("$w$");
fillRuv("$uv$");
fillRvw("$vw$");
fillRuw("$uw$");
fillRuvw("$uvw$");
makeVenn("");
\end{asy}

==> VennDiagrams.tex <==

Case 1: 
        \begin{asy}
          fillRuv("$Y$");
          fillRvw("$Z$");
          makeVenn("Case 1");
        \end{asy}

Case 2: 
        \begin{asy}
          fillRuv("$Y$");
          fillRvw("$Z$");
          fillRuvw("$C$");
          makeVenn("Case 2");
        \end{asy}

Case 3: 
        \begin{asy}
          fillRuv("$Y$");
          fillRvw("$Z$");
          fillRuw("$M$");
          makeVenn("Case 3");
        \end{asy}

Case 4: 
        \begin{asy}
          fillRuv("$Y$");
          fillRvw("$Z$");
          fillRuw("$M$");
          fillRuvw("$C$");
          makeVenn("Case 4");
        \end{asy}

Case 5: 
         \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          makeVenn("Case 5");
        \end{asy}

Case 6: 
        \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          fillRuvw("$C$");
          makeVenn("Case 6");
        \end{asy}

Case 7: 
         \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          fillRvw("$Z$");
          makeVenn("Case 7");
        \end{asy}

Case 8: 
        \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          fillRvw("$Z$");
          fillRuvw("$C$");
          makeVenn("Case 8");
        \end{asy}

Case 9: 
         \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          fillRuw("$Z$");
          makeVenn("Case 9");
        \end{asy}

Case 10: 
        \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          fillRuw("$Z$");
          fillRuvw("$C$");
          makeVenn("Case 10");
        \end{asy}

Case 11: 
         \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          fillRvw("$Z$");
          fillRuw("$M$");
          makeVenn("Case 11");
        \end{asy}

Case 12: 
        \begin{asy}
          fillRu("$X$");
          fillRuv("$Y$");
          fillRvw("$Z$");
          fillRuw("$M$");
          fillRuvw("$C$");
          makeVenn("Case 12");
        \end{asy}
